Deep Bayes Factor Scoring for Authorship Verification

The PAN 2020 authorship verification (AV) challenge focuses on a cross-topic/closed-set AV task over a collection of fanfiction texts. Fanfiction is a fan-written extension of a storyline in which a so-called fandom topic describes the principal subject of the document. The data provided in the PAN 2020 AV task is quite challenging because authors of texts across multiple/different fandom topics are included. In this work, we present a hierarchical fusion of two well-known approaches into a single end-to-end learning procedure: A deep metric learning framework at the bottom aims to learn a pseudo-metric that maps a document of variable length onto a fixed-sized feature vector. At the top, we incorporate a probabilistic layer to perform Bayes factor scoring in the learned metric space. We also provide text preprocessing strategies to deal with the cross-topic issue.

==> sections/doc.tex <==
{\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{11cm}{
\colorbox{blue!76.41161}{\strut ~~~}\colorbox{red!0.4193917}{\strut <HarryPotter>} \colorbox{red!0.53467476}{\strut '} \colorbox{red!0.61363894}{\strut What} \colorbox{red!0.6430992}{\strut on} \colorbox{red!0.6396857}{\strut Earth} \colorbox{red!0.7209753}{\strut are} \colorbox{red!0.6172148}{\strut you} \colorbox{red!2.5320923}{\strut doing} \colorbox{red!4.5420475}{\strut running} \colorbox{red!3.4149885}{\strut through} \colorbox{red!1.3643258}{\strut the} \colorbox{red!19.74599}{\strut halls} \colorbox{red!1.3197281}{\strut at} \colorbox{red!5.666561}{\strut almost} \colorbox{red!47.667244}{\strut 10:30} \colorbox{red!1.1859703}{\strut at} \colorbox{red!5.073587}{\strut night} \colorbox{red!1.9597912}{\strut ,} \colorbox{red!22.513031}{\strut Mr} \colorbox{red!7.1938505}{\strut Potter} \colorbox{red!1.0740887}{\strut ?} \colorbox{red!0.6629163}{\strut '} \colorbox{red!3.0602798}{\strut Severus} \colorbox{red!7.737382}{\strut asked} \colorbox{red!1.6655192}{\strut ,} \colorbox{red!7.532089}{\strut reaching} \colorbox{red!1.6343727}{\strut down} \colorbox{red!1.0114777}{\strut to} \colorbox{red!1.3326392}{\strut help} \colorbox{red!1.515547}{\strut lift} 
 \newline\colorbox{blue!91.828575}{\strut ~~~}\colorbox{red!1.0831435}{\strut <HarryPotter>} \colorbox{red!1.2177814}{\strut down} \colorbox{red!1.0740334}{\strut to} \colorbox{red!1.4970616}{\strut help} \colorbox{red!3.33996}{\strut lift} \colorbox{red!1.4606357}{\strut Harry} \colorbox{red!1.4083827}{\strut .} \colorbox{red!1.9780731}{\strut Harry} \colorbox{red!30.752293}{\strut flinched} \colorbox{red!1.6005967}{\strut ,} \colorbox{red!4.2859282}{\strut and} \colorbox{red!7.472821}{\strut then} \colorbox{red!16.676203}{\strut stared} \colorbox{red!1.2390633}{\strut at} \colorbox{red!3.6615956}{\strut Severus} \colorbox{red!1.1382729}{\strut '} \colorbox{red!23.238184}{\strut offered} \colorbox{red!2.8313105}{\strut hand} \colorbox{red!1.5701743}{\strut in} \colorbox{red!18.593077}{\strut surprise} \colorbox{red!1.1095228}{\strut .} \colorbox{red!4.5050282}{\strut When} \colorbox{red!1.2583385}{\strut he} \colorbox{red!8.852028}{\strut glanced} \colorbox{red!0.8975287}{\strut up} \colorbox{red!1.1189996}{\strut to} \colorbox{red!3.530548}{\strut Severus} \colorbox{red!1.3949733}{\strut '} \colorbox{red!5.1730347}{\strut face} \colorbox{red!1.6356257}{\strut ,} 
 \newline\colorbox{blue!66.95604}{\strut ~~~}\colorbox{red!1.3243732}{\strut <HarryPotter>} \colorbox{red!2.0670762}{\strut Severus} \colorbox{red!1.7318763}{\strut '} \colorbox{red!3.2763298}{\strut face} \colorbox{red!1.8295627}{\strut ,} \colorbox{red!1.5555187}{\strut his} \colorbox{red!17.5608}{\strut eyebrows} \colorbox{red!1.5390868}{\strut were} \colorbox{red!11.978486}{\strut raised} \colorbox{red!4.0141554}{\strut and} \colorbox{red!1.970242}{\strut his} \colorbox{red!3.8149264}{\strut eyes} \colorbox{red!2.133761}{\strut were} \colorbox{red!16.068773}{\strut guarded} \colorbox{red!0.9751325}{\strut .} \colorbox{red!1.8568169}{\strut Harry} \colorbox{red!4.2518096}{\strut took} \colorbox{red!1.7331645}{\strut the} \colorbox{red!18.032654}{\strut offered} \colorbox{red!3.5075266}{\strut hand} \colorbox{red!2.6097066}{\strut ,} \colorbox{red!19.290794}{\strut leaning} \colorbox{red!1.2828561}{\strut on} \colorbox{red!1.3936474}{\strut it} \colorbox{red!1.5596251}{\strut as} \colorbox{red!1.406302}{\strut he} \colorbox{red!3.1144938}{\strut got} \colorbox{red!1.2181915}{\strut up} \colorbox{red!1.3389047}{\strut ,} \colorbox{red!21.157606}{\strut wincing} 
 \newline\colorbox{blue!75.05932}{\strut ~~~}\colorbox{red!1.2190294}{\strut <HarryPotter>} \colorbox{red!1.8464333}{\strut got} \colorbox{red!1.4356025}{\strut up} \colorbox{red!1.4364074}{\strut ,} \colorbox{red!47.725113}{\strut wincing} \colorbox{red!1.4462}{\strut as} \colorbox{red!1.5823524}{\strut he} \colorbox{red!8.001865}{\strut put} \colorbox{red!13.124092}{\strut weight} \colorbox{red!1.3656499}{\strut on} \colorbox{red!1.4776363}{\strut his} \colorbox{red!3.0655355}{\strut leg} \colorbox{red!1.1431993}{\strut .} \colorbox{red!0.8372257}{\strut '} \colorbox{red!1.0977864}{\strut I} \colorbox{red!4.6946917}{\strut heard} \colorbox{red!6.1837835}{\strut something} \colorbox{red!1.3016411}{\strut ,} \colorbox{red!0.87103283}{\strut '} \colorbox{red!1.7974033}{\strut Harry} \colorbox{red!9.915845}{\strut said} \colorbox{red!3.410791}{\strut ,} \colorbox{red!23.529158}{\strut looking} \colorbox{red!4.4530196}{\strut around} \colorbox{red!1.3781039}{\strut .} \colorbox{red!1.0515777}{\strut '} \colorbox{red!1.7580175}{\strut You} \colorbox{red!3.429312}{\strut did} \colorbox{red!2.571568}{\strut n't} \colorbox{red!2.4441383}{\strut see} 
 \newline\colorbox{blue!58.995564}{\strut ~~~}\colorbox{red!0.67083734}{\strut <HarryPotter>} \colorbox{red!0.7059696}{\strut You} \colorbox{red!1.4929224}{\strut did} \colorbox{red!1.2528467}{\strut n't} \colorbox{red!1.3526675}{\strut see} \colorbox{red!3.918308}{\strut anyone} \colorbox{red!1.1625645}{\strut ,} \colorbox{red!2.2940397}{\strut did} \colorbox{red!1.1383255}{\strut you} \colorbox{red!1.1231433}{\strut ?} \colorbox{red!0.9824953}{\strut '} \colorbox{red!2.0516088}{\strut He} \colorbox{red!10.580157}{\strut asked} \colorbox{red!1.3049165}{\strut .} \colorbox{red!1.2217398}{\strut '} \colorbox{red!22.426018}{\strut Except} \colorbox{red!3.2057662}{\strut for} \colorbox{red!1.6627433}{\strut my} \colorbox{red!4.180881}{\strut son} \colorbox{red!17.562191}{\strut falling} \colorbox{red!2.1749127}{\strut at} \colorbox{red!1.998277}{\strut my} \colorbox{red!18.469284}{\strut feet} \colorbox{red!4.116846}{\strut ,} \colorbox{red!15.917715}{\strut half} \colorbox{red!2.0735836}{\strut an} \colorbox{red!3.7376542}{\strut hour} \colorbox{red!6.5639405}{\strut after} \colorbox{red!18.886105}{\strut curfew} \colorbox{red!1.3657206}{\strut no} 
 \newline\colorbox{blue!80.97735}{\strut ~~~}\colorbox{red!0.5480937}{\strut <HarryPotter>} \colorbox{red!0.6662489}{\strut hour} \colorbox{red!1.2389022}{\strut after} \colorbox{red!4.2870646}{\strut curfew} \colorbox{red!0.69789535}{\strut no} \colorbox{red!1.8621484}{\strut less} \colorbox{red!0.58833313}{\strut ?} \colorbox{red!0.5813016}{\strut No} \colorbox{red!0.68491393}{\strut ,} \colorbox{red!0.53187215}{\strut I} \colorbox{red!1.286701}{\strut did} \colorbox{red!1.0377605}{\strut not} \colorbox{red!0.8659701}{\strut ,} \colorbox{red!0.61069846}{\strut '} \colorbox{red!2.748413}{\strut Severus} \colorbox{red!10.659267}{\strut answered} \colorbox{red!0.8599068}{\strut .} \colorbox{red!1.399315}{\strut Harry} \colorbox{red!30.47308}{\strut shivered} \colorbox{red!1.5172539}{\strut as} \colorbox{red!1.3255143}{\strut the} \colorbox{red!5.5639396}{\strut wind} \colorbox{red!46.9233}{\strut whistled} \colorbox{red!7.5108647}{\strut through} \colorbox{red!1.5150518}{\strut the} \colorbox{red!18.738495}{\strut hallway} \colorbox{red!3.7513695}{\strut and} \colorbox{red!3.9986014}{\strut turned} \colorbox{red!1.1612617}{\strut his} \colorbox{red!1.9606531}{\strut head} 
 \newline\colorbox{blue!40.208702}{\strut ~~~}\colorbox{red!1.0912298}{\strut <HarryPotter>} \colorbox{red!1.615699}{\strut and} \colorbox{red!2.1862226}{\strut turned} \colorbox{red!1.134684}{\strut his} \colorbox{red!2.0492651}{\strut head} \colorbox{red!8.228782}{\strut towards} \colorbox{red!1.1580435}{\strut the} \colorbox{red!2.8724089}{\strut noise} \colorbox{red!0.87066096}{\strut .} \colorbox{red!0.6834268}{\strut '} \colorbox{red!1.6818146}{\strut What} \colorbox{red!2.302682}{\strut did} \colorbox{red!1.0977955}{\strut it} \colorbox{red!2.8517573}{\strut sound} \colorbox{red!1.4884423}{\strut like} \colorbox{red!0.7261646}{\strut ?} \colorbox{red!0.72972345}{\strut '} \colorbox{red!0.85351413}{\strut '} \colorbox{red!10.506611}{\strut Something} \colorbox{red!1.6933447}{\strut was} \colorbox{red!12.61794}{\strut saying} \colorbox{red!1.1621767}{\strut '} \colorbox{red!4.0539393}{\strut kill} \colorbox{red!2.520032}{\strut ,} \colorbox{red!27.064287}{\strut rip} \colorbox{red!1.8762267}{\strut ,} \colorbox{red!50.98787}{\strut maim} \colorbox{red!0.8613691}{\strut '} \colorbox{red!6.8291044}{\strut over} \colorbox{red!1.7989744}{\strut and} 
 \newline\colorbox{blue!38.008152}{\strut ~~~}\colorbox{red!1.2874874}{\strut <HarryPotter>} \colorbox{red!51.13236}{\strut maim} \colorbox{red!1.5480188}{\strut '} \colorbox{red!10.281257}{\strut over} \colorbox{red!3.5070593}{\strut and} \colorbox{red!6.2152114}{\strut over} \colorbox{red!5.714305}{\strut again} \colorbox{red!1.7429382}{\strut in} \colorbox{red!2.091817}{\strut ,} \colorbox{red!2.7684038}{\strut like} \colorbox{red!1.9898107}{\strut ,} \colorbox{red!1.6161062}{\strut a} \colorbox{red!7.785094}{\strut whisper} \colorbox{red!1.2772536}{\strut .} \colorbox{red!8.195505}{\strut Except} \colorbox{red!1.168819}{\strut it} \colorbox{red!1.723564}{\strut was} \colorbox{red!5.251785}{\strut really} \colorbox{red!7.656385}{\strut loud} \colorbox{red!1.4373593}{\strut .} \colorbox{red!7.16108}{\strut Like} \colorbox{red!4.0933814}{\strut nothing} \colorbox{red!1.4300947}{\strut I} \colorbox{red!3.0560362}{\strut 've} \colorbox{red!5.163062}{\strut ever} \colorbox{red!2.9038296}{\strut heard} \colorbox{red!3.2617145}{\strut before} \colorbox{red!1.0539303}{\strut ,} \colorbox{red!1.1381694}{\strut '} \colorbox{red!1.9423949}{\strut Harry} 
 \newline\colorbox{blue!88.24355}{\strut ~~~}\colorbox{red!0.6731941}{\strut <HarryPotter>} \colorbox{red!1.0931561}{\strut before} \colorbox{red!0.50060993}{\strut ,} \colorbox{red!0.44645056}{\strut '} \colorbox{red!0.96542674}{\strut Harry} \colorbox{red!4.4530115}{\strut said} \colorbox{red!1.7223272}{\strut ,} \colorbox{red!16.134178}{\strut rubbing} \colorbox{red!1.3467919}{\strut at} \colorbox{red!1.4580978}{\strut his} \colorbox{red!10.6171}{\strut forehead} \colorbox{red!0.8821451}{\strut .} \colorbox{red!3.7043657}{\strut Severus} \colorbox{red!54.609806}{\strut regarded} \colorbox{red!1.8089099}{\strut him} \colorbox{red!2.5946493}{\strut for} \colorbox{red!1.4004616}{\strut a} \colorbox{red!16.410627}{\strut moment} \colorbox{red!5.1758904}{\strut before} \colorbox{red!9.201958}{\strut saying} \colorbox{red!1.3477619}{\strut ,} \colorbox{red!0.7614032}{\strut '} \colorbox{red!7.3324957}{\strut Are} \colorbox{red!1.2353444}{\strut you} \colorbox{red!2.6796334}{\strut sure} \colorbox{red!0.988072}{\strut it} \colorbox{red!1.2021332}{\strut was} \colorbox{red!1.661309}{\strut n't} \colorbox{red!0.9883147}{\strut the} \colorbox{red!2.1985748}{\strut wind} 
 \newline\colorbox{blue!30.426413}{\strut ~~~}\colorbox{red!2.368672}{\strut <HarryPotter>} \colorbox{red!2.781784}{\strut was} \colorbox{red!2.9035141}{\strut n't} \colorbox{red!2.8290913}{\strut the} \colorbox{red!6.954996}{\strut wind} \colorbox{red!2.613506}{\strut ?} \colorbox{red!8.757555}{\strut At} \colorbox{red!4.664796}{\strut night} \colorbox{red!3.2094295}{\strut ,} \colorbox{red!2.991245}{\strut in} \colorbox{red!3.5874891}{\strut an} \colorbox{red!9.855536}{\strut unfamiliar} \colorbox{red!4.0399814}{\strut part} \colorbox{red!2.4849946}{\strut of} \colorbox{red!2.4225621}{\strut the} \colorbox{red!3.0635753}{\strut castle} \colorbox{red!2.0015337}{\strut ,} \colorbox{red!2.3645124}{\strut your} \colorbox{red!2.5845344}{\strut brain} \colorbox{red!1.9723401}{\strut can} \colorbox{red!3.1043894}{\strut play} \colorbox{red!23.432196}{\strut tricks} \colorbox{red!3.7447739}{\strut on} \colorbox{red!3.5292716}{\strut you} \colorbox{red!2.924166}{\strut .} \colorbox{red!2.8217185}{\strut '} \colorbox{red!4.127368}{\strut Harry} \colorbox{red!24.85897}{\strut fixed} \colorbox{red!5.140526}{\strut him} \colorbox{red!7.45916}{\strut with} 
 \newline\colorbox{blue!51.471256}{\strut ~~~}\colorbox{red!1.4876273}{\strut <HarryPotter>} \colorbox{red!1.5224117}{\strut Harry} \colorbox{red!8.59543}{\strut fixed} \colorbox{red!2.1000621}{\strut him} \colorbox{red!3.377735}{\strut with} \colorbox{red!1.7299314}{\strut a} \colorbox{red!14.695981}{\strut glare} \colorbox{red!2.797807}{\strut and} \colorbox{red!10.199413}{\strut shook} \colorbox{red!1.777735}{\strut his} \colorbox{red!4.0073175}{\strut head} \colorbox{red!1.3118397}{\strut .} \colorbox{red!1.2665324}{\strut '} \colorbox{red!2.2044272}{\strut No} \colorbox{red!2.277348}{\strut ,} \colorbox{red!1.5235753}{\strut I} \colorbox{red!1.5602336}{\strut 'm} \colorbox{red!2.5281608}{\strut not} \colorbox{red!9.300162}{\strut imagining} \colorbox{red!1.3388646}{\strut it} \colorbox{red!1.5335604}{\strut ,} \colorbox{red!1.054543}{\strut '} \colorbox{red!2.0728896}{\strut Harry} \colorbox{red!9.222305}{\strut said} \colorbox{red!3.4719694}{\strut ,} \colorbox{red!19.493208}{\strut resisting} \colorbox{red!2.2985363}{\strut the} \colorbox{red!16.945482}{\strut urge} \colorbox{red!2.0855856}{\strut to} \colorbox{red!21.81354}{\strut mutter} 
 \newline\colorbox{blue!47.134674}{\strut ~~~}\colorbox{red!1.4745888}{\strut <HarryPotter>} \colorbox{red!1.3193486}{\strut the} \colorbox{red!5.348839}{\strut urge} \colorbox{red!1.2379943}{\strut to} \colorbox{red!15.85843}{\strut mutter} \colorbox{red!1.585643}{\strut that} \colorbox{red!1.5114392}{\strut he} \colorbox{red!1.6790775}{\strut was} \colorbox{red!2.2646506}{\strut n't} \colorbox{red!8.993519}{\strut imagining} \colorbox{red!1.492551}{\strut the} \colorbox{red!4.189446}{\strut stuff} \colorbox{red!2.051341}{\strut with} \colorbox{red!15.506485}{\strut Lockhart} \colorbox{red!10.03167}{\strut either} \colorbox{red!0.84599096}{\strut .} \colorbox{red!0.9087934}{\strut '} \colorbox{red!9.072387}{\strut Very} \colorbox{red!5.775089}{\strut well} \colorbox{red!1.2728496}{\strut .} \colorbox{red!1.5097669}{\strut I} \colorbox{red!2.8233182}{\strut will} \colorbox{red!33.309113}{\strut inform} \colorbox{red!1.7807772}{\strut the} \colorbox{red!8.274595}{\strut Headmaster} \colorbox{red!1.5880592}{\strut ,} \colorbox{red!5.927224}{\strut though} \colorbox{red!0.933144}{\strut it} \colorbox{red!3.8301554}{\strut quite} \colorbox{red!3.1978812}{\strut possibly} 
 \newline\colorbox{blue!40.913082}{\strut ~~~}\colorbox{red!3.1398945}{\strut <HarryPotter>} \colorbox{red!3.0247855}{\strut though} \colorbox{red!3.2544777}{\strut it} \colorbox{red!5.748876}{\strut quite} \colorbox{red!7.8553267}{\strut possibly} \colorbox{red!4.2485833}{\strut was} \colorbox{red!5.864315}{\strut just} \colorbox{red!5.214294}{\strut Peeves} \colorbox{red!10.302672}{\strut playing} \colorbox{red!3.4948642}{\strut a} \colorbox{red!11.916067}{\strut nasty} \colorbox{red!10.673464}{\strut joke} \colorbox{red!4.9155025}{\strut .} \colorbox{red!5.805559}{\strut Why} \colorbox{red!5.0066323}{\strut are} \colorbox{red!4.2338467}{\strut you} \colorbox{red!3.6545768}{\strut up} \colorbox{red!4.991988}{\strut here} \colorbox{red!4.0016723}{\strut so} \colorbox{red!8.701914}{\strut late} \colorbox{red!5.147104}{\strut ,} \colorbox{red!5.2018194}{\strut Harry} \colorbox{red!4.4384775}{\strut ?} \colorbox{red!3.3888016}{\strut Your} \colorbox{red!3.4370384}{\strut detention} \colorbox{red!2.969069}{\strut should} \colorbox{red!3.6217797}{\strut have} \colorbox{red!4.351595}{\strut finished} \colorbox{red!2.9625278}{\strut hours} \colorbox{red!4.0266695}{\strut ago} 
 \newline\colorbox{blue!40.68343}{\strut ~~~}\colorbox{red!1.537443}{\strut <HarryPotter>} \colorbox{red!1.8532889}{\strut have} \colorbox{red!2.4940317}{\strut finished} \colorbox{red!1.6173128}{\strut hours} \colorbox{red!1.94226}{\strut ago} \colorbox{red!1.2252213}{\strut ,} \colorbox{red!1.1144563}{\strut '} \colorbox{red!4.367537}{\strut Severus} \colorbox{red!13.16398}{\strut asked} \colorbox{red!1.9051814}{\strut .} \colorbox{red!2.935607}{\strut Harry} \colorbox{red!19.11303}{\strut looked} \colorbox{red!2.8304977}{\strut up} \colorbox{red!2.3829746}{\strut at} \colorbox{red!3.1142616}{\strut him} \colorbox{red!4.0376515}{\strut ,} \colorbox{red!19.254797}{\strut wondering} \colorbox{red!6.4240932}{\strut what} \colorbox{red!2.9426196}{\strut he} \colorbox{red!20.830648}{\strut meant} \colorbox{red!2.4205713}{\strut .} \colorbox{red!2.0593297}{\strut '} \colorbox{red!2.4725885}{\strut You} \colorbox{red!4.3639517}{\strut always} \colorbox{red!4.0105414}{\strut keep} \colorbox{red!1.7798934}{\strut me} \colorbox{red!2.3727314}{\strut until} \colorbox{red!3.1115534}{\strut almost} \colorbox{red!15.930051}{\strut curfew} \colorbox{red!1.9861116}{\strut .} 
 \newline\colorbox{blue!45.090717}{\strut ~~~}\colorbox{red!0.7828905}{\strut <HarryPotter>} \colorbox{red!0.8825563}{\strut until} \colorbox{red!1.4066823}{\strut almost} \colorbox{red!9.372671}{\strut curfew} \colorbox{red!0.8400769}{\strut .} \colorbox{red!13.439734}{\strut Lockhart} \colorbox{red!3.0036056}{\strut said} \colorbox{red!1.3131073}{\strut he} \colorbox{red!7.1324835}{\strut lost} \colorbox{red!9.420094}{\strut track} \colorbox{red!1.5225645}{\strut of} \colorbox{red!3.460067}{\strut time} \colorbox{red!1.1151528}{\strut .} \colorbox{red!3.8636346}{\strut And} \colorbox{red!1.0329665}{\strut I} \colorbox{red!3.3021011}{\strut fell} \colorbox{red!8.283672}{\strut asleep} \colorbox{red!1.9418035}{\strut ,} \colorbox{red!26.170343}{\strut anyway} \colorbox{red!1.0290009}{\strut ,} \colorbox{red!0.5927517}{\strut '} \colorbox{red!1.4657812}{\strut Harry} \colorbox{red!43.32014}{\strut admitted} \colorbox{red!1.0864975}{\strut .} \colorbox{red!1.0133332}{\strut '} \colorbox{red!1.2299118}{\strut I} \colorbox{red!3.1224205}{\strut keep} \colorbox{red!0.9988649}{\strut you} \colorbox{red!1.5665574}{\strut until} \colorbox{red!1.8827441}{\strut almost} 
 \newline
}}}

